PyRelationAL: a python library for active learning research and development

Active learning (AL) is a sub-field of ML focused on the development of methods to iteratively and economically acquire data by strategically querying new data points that are the most useful for a particular task. Here, we introduce PyRelationAL, an open source library for AL research. We describe a modular toolkit based around a two step design methodology for composing pool-based active learning strategies applicable to both single-acquisition and batch-acquisition strategies. This framework allows for the mathematical and practical specification of a broad number of existing and novel strategies under a consistent programming model and abstraction. Furthermore, we incorporate datasets and active learning tasks applicable to them to simplify comparative evaluation and benchmarking, along with an initial group of benchmarks across datasets included in this library. The toolkit is compatible with existing ML frameworks. PyRelationAL is maintained using modern software engineering practices -- with an inclusive contributor code of conduct -- to promote long term library quality and utilisation. PyRelationAL is available under a permissive Apache licence on PyPi and at https://github.com/RelationRx/pyrelational.

==> code_snippets/updated_run_with_pipeline.tex <==
\begin{code}


\begin{minted}[linenos,fontsize=\small,xleftmargin=0.5cm,numbersep=3pt,frame=lines]{python}
from pyrelational.oracles import BenchmarkOracle
from pyrelational.pipeline import Pipeline

# A Pipeline is a composition of DataManager, 
# ModelManager, Strategy, and Oracle objects
data_manager = get_data_manager()
model_manager = TorchEnsembleWrapper(
    DiabetesRegression,
    {"dropout": 0.12},
    {"epochs":100, "lr":3e-4},
    n_estimators=10,
)
strategy = EpsilonGreedyStrategy(eps=0.05)
oracle = BenchmarkOracle()
pipeline = Pipeline(
    data_manager = data_manager,
    model_manager = model_manager,
    strategy = strategy,
    oracle = oracle,
)

# New data to be annotated, followed by an update of the data_manager and model
to_annotate = pipeline.step(num_annotate=25)
pipeline.query(indices=to_annotate)

# Annotating data step by step until the trainset is fully annotated
pipeline.run(num_annotate=25)
\end{minted}
\captionof{listing}{Integrating each of the custom data manager, ensemble of models, and strategy into a pipeline along with an oracle for benchmarking strategies. After a pipeline is instantiated we may iterate on the active learning cycle.}\label{code:updated_run_with_pipeline}
\end{code}
